The Hybrid Bootstrap: A Drop-in Replacement for Dropout

Regularization is an important component of predictive model building. The hybrid bootstrap is a regularization technique that functions similarly to dropout except that features are resampled from other training points rather than replaced with zeros. We show that the hybrid bootstrap offers superior performance to dropout. We also present a sampling based technique to simplify hyperparameter choice. Next, we provide an alternative sampling technique for convolutional neural networks. Finally, we demonstrate the efficacy of the hybrid bootstrap on non-image tasks using tree-based models.

==> refs.tex <==
@book{goodfellow2016deep,
  title={Deep Learning},
  author={Goodfellow, Ian and Bengio, Yoshua and Courville, Aaron},
  year={2016},
  publisher={MIT Press}
}

@article{srivastava2014dropout,
  title={Dropout: a simple way to prevent neural networks from overfitting.},
  author={Srivastava, Nitish and Hinton, Geoffrey E and Krizhevsky, Alex and Sutskever, Ilya and Salakhutdinov, Ruslan},
  journal={Journal of Machine Learning Research},
  volume={15},
  number={1},
  pages={1929--1958},
  year={2014}
}

@inproceedings{wager2013dropout,
  title={Dropout training as adaptive regularization},
  author={Wager, Stefan and Wang, Sida and Liang, Percy S},
  booktitle={Advances in Neural Information Processing Systems},
  pages={351--359},
  year={2013}
}

@article{sietsma1991creating,
  title={Creating artificial neural networks that generalize},
  author={Sietsma, Jocelyn and Dow, Robert JF},
  journal={Neural Networks},
  volume={4},
  number={1},
  pages={67--79},
  year={1991},
  publisher={Elsevier}
}

@article{bishop1995training,
  title={Training with noise is equivalent to {T}ikhonov regularization},
  author={Bishop, Chris M},
  journal={Neural Computation},
  volume={7},
  number={1},
  pages={108--116},
  year={1995},
  publisher={MIT Press}
}

@inproceedings{van2013learning,
  title={Learning with Marginalized Corrupted Features.},
  author={Van Der Maaten, Laurens and Chen, Minmin and Tyree, Stephen and Weinberger, Kilian Q},
  booktitle={Proceedings of the 30th International Conference on Machine Learning},
  pages={410--418},
  year={2013}
}

@book{goodfellow2016deep,
  title={Deep learning},
  author={Goodfellow, Ian and Bengio, Yoshua and Courville, Aaron},
  year={2016},
  pages={233--234}
  publisher={MIT Press}
}

@article{lecun1998gradient,
  title={Gradient-based learning applied to document recognition},
  author={LeCun, Yann and Bottou, L{\'e}on and Bengio, Yoshua and Haffner, Patrick},
  journal={Proceedings of the IEEE},
  volume={86},
  number={11},
  pages={2278--2324},
  year={1998},
  publisher={IEEE}
}

@inproceedings{wan2013regularization,
  title={Regularization of neural networks using {DropConnect}},
  author={Wan, Li and Zeiler, Matthew and Zhang, Sixin and Cun, Yann L and Fergus, Rob},
  booktitle={Proceedings of the 30th International Conference on Machine Learning},
  pages={1058--1066},
  year={2013}
}

@inproceedings{globerson2006nightmare,
  title={Nightmare at test time: robust learning by feature deletion},
  author={Globerson, Amir and Roweis, Sam},
  booktitle={Proceedings of the 23rd International Conference on Machine Learning},
  pages={353--360},
  year={2006},
  organization={ACM}
}

@book{efron1994introduction,
  title={An Introduction to the Bootstrap},
  author={Efron, Bradley and Tibshirani, Robert J},
  year={1994},
  publisher={CRC press}
}

@article{lecun1989backpropagation,
  title={Backpropagation applied to handwritten zip code recognition},
  author={LeCun, Yann and Boser, Bernhard and Denker, John S and Henderson, Donnie and Howard, Richard E and Hubbard, Wayne and Jackel, Lawrence D},
  journal={Neural Computation},
  volume={1},
  number={4},
  pages={541--551},
  year={1989},
  publisher={MIT Press}
}

@article{friedman2001greedy,
  title={Greedy function approximation: a gradient boosting machine},
  author={Friedman, Jerome H},
  journal={Annals of statistics},
  pages={1189--1232},
  year={2001},
  publisher={JSTOR}
}

@techreport{rosenblatt1961principles,
  title={Principles of neurodynamics. perceptrons and the theory of brain mechanisms},
  author={Rosenblatt, Frank},
  year={1961},
  institution={DTIC Document}
}

@inproceedings{nair2010rectified,
  title={Rectified linear units improve restricted {B}oltzmann machines},
  author={Nair, Vinod and Hinton, Geoffrey E},
  booktitle={Proceedings of the 27th International Conference on Machine Learning (ICML-10)},
  pages={807--814},
  year={2010}
}

@misc{chollet2015keras,
  title={Keras},
  author={Chollet, Fran\c{c}ois and others},
  year={2015},
  publisher={GitHub},
  howpublished={\url{https://github.com/fchollet/keras}},
}

@ARTICLE{2016arXiv160502688short,
   author = {{Theano Development Team}},
    title = "{Theano: A {Python} framework for fast computation of mathematical expressions}",
  journal = {arXiv e-prints},
   volume = {abs/1605.02688},
 primaryClass = "cs.SC",
 keywords = {Computer Science - Symbolic Computation, Computer Science - Learning, Computer Science - Mathematical Software},
     year = 2016,
    month = may,
      url = {http://arxiv.org/abs/1605.02688},
}

@inproceedings{tompson2015efficient,
  title={Efficient object localization using convolutional networks},
  author={Tompson, Jonathan and Goroshin, Ross and Jain, Arjun and LeCun, Yann and Bregler, Christoph},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={648--656},
  year={2015}
}

@inproceedings{chen2016xgboost,
  title={{XGBoost}: A scalable tree boosting system},
  author={Chen, Tianqi and Guestrin, Carlos},
  booktitle={Proceedings of the 22nd ACM SIGKDD International Conference on Knowledge Discovery and Data Mining},
  pages={785--794},
  year={2016},
  organization={ACM}
}

@inproceedings{street1993nuclear,
  title={Nuclear feature extraction for breast tumor diagnosis},
  author={Street, W Nick and Wolberg, William H and Mangasarian, Olvi L},
  booktitle={Biomedical Image Processing and Biomedical Visualization},
  volume={1905},
  pages={861--871},
  year={1993},
  organization={International Society for Optics and Photonics}
}

@InProceedings{pmlr-v38-korlakaivinayak15,
  title = 	 {{DART: Dropouts meet Multiple Additive Regression Trees}},
  author = 	 {Rashmi Korlakai Vinayak and Ran Gilad-Bachrach},
  booktitle = 	 {Proceedings of the Eighteenth International Conference on Artificial Intelligence and Statistics},
  pages = 	 {489--497},
  year = 	 {2015}
}

@INPROCEEDINGS{Zagoruyko2016WRN,
    author = {Sergey Zagoruyko and Nikos Komodakis},
    title = {Wide Residual Networks},
    booktitle = {BMVC},
    year = {2016}}

@article{krizhevsky2009learning,
  title={Learning multiple layers of features from tiny images},
  author={Krizhevsky, Alex and Hinton, Geoffrey},
  year={2009},
  journal={Technical report, University of Toronto}
}


@misc{titanic,
  title = {{titanic3 Data Description}},
  howpublished = {\url{http://biostat.mc.vanderbilt.edu/wiki/pub/Main/DataSets/titanic3info.txt} [Accessed: 2018-01-01]},
  author = {Cason, Thomas}
}

@ARTICLE{convex1,
   author = {{Zhang}, H. and {Cisse}, M. and {Dauphin}, Y.~N. and {Lopez-Paz}, D.
	},
    title = "{mixup: Beyond Empirical Risk Minimization}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1710.09412},
 primaryClass = "cs.LG",
 keywords = {Computer Science - Learning, Statistics - Machine Learning},
     year = 2017,
    month = oct,
   adsurl = {http://adsabs.harvard.edu/abs/2017arXiv171009412Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{convex2,
   author = {{Tokozume}, Y. and {Ushiku}, Y. and {Harada}, T.},
    title = "{Between-class Learning for Image Classification}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1711.10284},
 primaryClass = "cs.LG",
 keywords = {Computer Science - Learning, Computer Science - Computer Vision and Pattern Recognition, Statistics - Machine Learning},
     year = 2017,
    month = nov,
   adsurl = {http://adsabs.harvard.edu/abs/2017arXiv171110284T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{convex3,
   author = {{Inoue}, H.},
    title = "{Data Augmentation by Pairing Samples for Images Classification}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1801.02929},
 primaryClass = "cs.LG",
 keywords = {Computer Science - Learning, Computer Science - Computer Vision and Pattern Recognition, Statistics - Machine Learning},
     year = 2018,
    month = jan,
   adsurl = {http://adsabs.harvard.edu/abs/2018arXiv180102929I},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}







